Improving Forecasts for Heterogeneous Time Series by "Averaging", with Application to Food Demand Forecast

A common forecasting setting in real world applications considers a set of possibly heterogeneous time series of the same domain. Due to different properties of each time series such as length, obtaining forecasts for each individual time series in a straight-forward way is challenging. This paper proposes a general framework utilizing a similarity measure in Dynamic Time Warping to find similar time series to build neighborhoods in a k-Nearest Neighbor fashion, and improve forecasts of possibly simple models by averaging. Several ways of performing the averaging are suggested, and theoretical arguments underline the usefulness of averaging for forecasting. Additionally, diagnostics tools are proposed allowing a deep understanding of the procedure.

==> paper_tables/multistep_eval.tex <==
\begin{table}

    \caption{\label{tab:multistep_mae}Multi-Step MAE (p-value 0.0112). The best results are in bold.}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}[t]{lrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{ } & \multicolumn{2}{c}{M3} & \multicolumn{2}{c}{CIF2016} & \multicolumn{2}{c}{HOSPITAL} & \multicolumn{2}{c}{TOURISM} \\
    \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9}
    Model & Mean & Median & Mean & Median & Mean & Median & Mean & Median\\
    \midrule
    TSAVG & 713.580 & 510.021 & \textbf{545365.6} & 98.162 & 21.440 & \textbf{6.763} & 7109.038 & 985.100\\
    ETS & 736.036 & 507.657 & 642448.9 & \textbf{90.546} & 22.553 & 6.782 & 7391.902 & 959.128\\
    ARIMA & \textbf{704.468} & \textbf{487.471} & 568230.7 & 105.003 & \textbf{20.665} & 6.869 & \textbf{4184.401} & \textbf{811.594}\\
    PLM-POOL & 1092.427 & 918.785 & 1300457.8 & 219661.126 & 26.370 & 11.247 & 8247.274 & 2585.891\\
    \bottomrule
    \end{tabular}}
    \end{table}
    \begin{table}
    
    \caption{\label{tab:multistep_rmse}Multi-Step RMSE (p-value 0.0112). The best results are in bold.}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}[t]{lrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{ } & \multicolumn{2}{c}{M3} & \multicolumn{2}{c}{CIF2016} & \multicolumn{2}{c}{HOSPITAL} & \multicolumn{2}{c}{TOURISM} \\
    \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9}
    Model & Mean & Median & Mean & Median & Mean & Median & Mean & Median\\
    \midrule
    TSAVG & 860.793 & 604.199 & \textbf{632468.5} & 117.239 & 26.225 & 8.347 & 8632.070 & 1241.053\\
    ETS & 886.086 & 626.804 & 722426.3 & \textbf{107.687} & 27.336 & 8.324 & 8974.416 & 1222.899\\
    ARIMA & \textbf{845.835} & \textbf{588.559} & 641597.5 & 126.505 & \textbf{25.021} & \textbf{8.241} & \textbf{5377.097} & \textbf{1090.481}\\
    PLM-POOL & 1279.612 & 1067.361 & 1456160.9 & 249604.091 & 31.425 & 13.006 & 10154.528 & 2954.635\\
    \bottomrule
    \end{tabular}}
    \end{table}
    \begin{table}
    
    \caption{\label{tab:multistep_rmsse}Multi-Step RMSSE (p-value 0.044). The best results are in bold.}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}[t]{lrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{ } & \multicolumn{2}{c}{M3} & \multicolumn{2}{c}{CIF2016} & \multicolumn{2}{c}{HOSPITAL} & \multicolumn{2}{c}{TOURISM} \\
    \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9}
    Model & Mean & Median & Mean & Median & Mean & Median & Mean & Median\\
    \midrule
    TSAVG & \textbf{1.915} & 1.178 & 1.121 & 0.864 & 0.878 & \textbf{0.822} & 1.761 & 1.468\\
    ETS & 1.967 & 1.220 & \textbf{1.105} & \textbf{0.809} & 0.900 & 0.828 & 1.853 & 1.497\\
    ARIMA & 1.927 & \textbf{1.108} & 1.191 & 0.896 & \textbf{0.871} & 0.822 & \textbf{1.597} & \textbf{1.414}\\
    PLM-POOL & 5.373 & 1.771 & 105106.814 & 2050.317 & 1.337 & 1.197 & 9.117 & 3.766\\
    \bottomrule
    \end{tabular}}
    \end{table}
    \begin{table}
    
    \caption{\label{tab:multistep_smape}Multi-Step sMAPE (p-value 0.044). The best results are in bold.}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}[t]{lrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{ } & \multicolumn{2}{c}{M3} & \multicolumn{2}{c}{CIF2016} & \multicolumn{2}{c}{HOSPITAL} & \multicolumn{2}{c}{TOURISM} \\
    \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9}
    Model & Mean & Median & Mean & Median & Mean & Median & Mean & Median\\
    \midrule
    TSAVG & \textbf{0.159} & 0.104 & 0.158 & \textbf{0.079} & 0.181 & 0.168 & 0.352 & 0.295\\
    ETS & 0.164 & 0.106 & \textbf{0.144} & 0.082 & 0.185 & \textbf{0.166} & 0.369 & 0.306\\
    ARIMA & 0.161 & \textbf{0.101} & 0.169 & 0.091 & \textbf{0.179} & 0.166 & \textbf{0.325} & \textbf{0.283}\\
    PLM-POOL & 0.232 & 0.174 & 1.726 & 1.970 & 0.219 & 0.190 & 0.746 & 0.644\\
    \bottomrule
    \end{tabular}}
    \end{table}

==> paper_tables/onestep_eval.tex <==
\begin{table}

    \caption{\label{tab:onestep_mae}Cumulative One-Step Ahead MAE (p-value 0.0503). The best results are in bold.}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}[t]{lrrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{ } & \multicolumn{2}{c}{M3} & \multicolumn{2}{c}{CIF2016} & \multicolumn{2}{c}{HOSPITAL} & \multicolumn{2}{c}{TOURISM} & \multicolumn{2}{c}{FOOD} \\
    \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9} \cmidrule(l{3pt}r{3pt}){10-11}
    Model & Mean & Median & Mean & Median & Mean & Median & Mean & Median & Mean & Median\\
    \midrule
    TSAVG & \textbf{484.660} & 322.573 & 301584.2 & 82.064 & 19.610 & \textbf{6.437} & 3647.229 & 770.753 & \textbf{8.523} & \textbf{6.917}\\
    ETS & 478.813 & 318.437 & 247264.0 & \textbf{76.378} & 19.635 & 6.491 & 3744.562 & 767.282 & 8.662 & 7.824\\
    ARIMA & 470.654 & \textbf{311.126} & \textbf{233306.1} & 79.007 & \textbf{19.040} & 6.495 & \textbf{3190.488} & \textbf{700.724} & 9.882 & 9.720\\
    PLM-POOL & 558.834 & 422.125 & 411428.1 & 32944.310 & 22.831 & 7.868 & 3976.333 & 863.865 & 9.438 & 7.387\\
    \bottomrule
    \end{tabular}}
    \end{table}
    \begin{table}
    
    \caption{\label{tab:onestep_rmse}Cumulative One-Step Ahead RMSE (p-value 0.0503). The best results are in bold.}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}[t]{lrrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{ } & \multicolumn{2}{c}{M3} & \multicolumn{2}{c}{CIF2016} & \multicolumn{2}{c}{HOSPITAL} & \multicolumn{2}{c}{TOURISM} & \multicolumn{2}{c}{FOOD} \\
    \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9} \cmidrule(l{3pt}r{3pt}){10-11}
    Model & Mean & Median & Mean & Median & Mean & Median & Mean & Median & Mean & Median\\
    \midrule
    TSAVG & 615.987 & 406.703 & 360462.5 & \textbf{93.481} & 23.985 & 8.080 & 4759.500 & 1005.795 & \textbf{10.112} & \textbf{8.417} \\
    ETS & 611.354 & 410.237 & 305246.7 & 93.493 & 23.991 & \textbf{7.992} & 4870.787 & 1008.100 & 10.193 & 8.720\\
    ARIMA & \textbf{598.826 }& \textbf{395.709} & \textbf{301763.1} & 96.834 & \textbf{23.320} & 8.022 & \textbf{4119.036} & \textbf{929.144} & 11.552 & 11.365\\
    PLM-POOL & 705.776 & 511.881 & 451571.8 & 32944.598 & 27.997 & 9.792 & 5278.082 & 1126.599 & 11.526 & 9.685\\
    \bottomrule
    \end{tabular}}
    \end{table}
    \begin{table}
    
    \caption{\label{tab:onestep_rmsse}Cumulative One-Step Ahead RMSSE (p-value 0.0189). The best results are in bold.}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}[t]{lrrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{ } & \multicolumn{2}{c}{M3} & \multicolumn{2}{c}{CIF2016} & \multicolumn{2}{c}{HOSPITAL} & \multicolumn{2}{c}{TOURISM} & \multicolumn{2}{c}{FOOD} \\
    \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9} \cmidrule(l{3pt}r{3pt}){10-11}
    Model & Mean & Median & Mean & Median & Mean & Median & Mean & Median & Mean & Median\\
    \midrule
    TSAVG & 0.904 & 0.805 & 0.885 & 0.802 & 0.824 & 0.800 & \textbf{1.418} & 1.320 & \textbf{0.875} & \textbf{0.748}\\
    ETS & 0.892 & 0.796 & \textbf{0.759} & 0.751 & \textbf{0.823} & 0.802 & 1.423 & 1.348 & 0.887 & 0.762\\
    ARIMA & \textbf{0.882} & \textbf{0.780} & 0.770 & \textbf{0.738} & 0.819 & \textbf{0.796} & 1.282 & \textbf{1.205} & 0.973 & 0.804\\
    PLM-POOL & 1.666 & 0.970 & 25562.026 & 280.377 & 1.010 & 0.978 & 1.926 & 1.713 & 1.354 & 0.939\\
    \bottomrule
    \end{tabular}}
    \end{table}
    \begin{table}
    
    \caption{\label{tab:onestep_smape}Cumulative One-Step Ahead sMAPE (p-value 0.0694). The best results are in bold.}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}[t]{lrrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{ } & \multicolumn{2}{c}{M3} & \multicolumn{2}{c}{CIF2016} & \multicolumn{2}{c}{HOSPITAL} & \multicolumn{2}{c}{TOURISM} & \multicolumn{2}{c}{FOOD} \\
    \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9} \cmidrule(l{3pt}r{3pt}){10-11}
    Model & Mean & Median & Mean & Median & Mean & Median & Mean & Median & Mean & Median\\
    \midrule
    TSAVG & 0.115 & 0.069 & 0.107 & 0.084 & \textbf{0.168} & \textbf{0.158} & 0.291 & 0.262 & \textbf{0.244} & \textbf{0.211}\\
    ETS & 0.114 & 0.068 & 0.097 & 0.082 & 0.169 & 0.160 & 0.288 & 0.265 & 0.251 & 0.214\\
    ARIMA & \textbf{0.114} & \textbf{0.065} & \textbf{0.101} & \textbf{0.080} & 0.169 & 0.161 & \textbf{0.267} & \textbf{0.241} & 0.301 & 0.242\\
    PLM-POOL & 0.132 & 0.079 & 1.589 & 1.882 & 0.184 & 0.175 & 0.361 & 0.297 & 0.274 & 0.230\\
    \bottomrule
    \end{tabular}}
    \end{table}
